CLAP: Learning Transferable Binary Code Representations with Natural Language Supervision

Binary code representation learning has shown significant performance in binary analysis tasks. But existing solutions often have poor transferability, particularly in few-shot and zero-shot scenarios where few or no training samples are available for the tasks. To address this problem, we present CLAP (Contrastive Language-Assembly Pre-training), which employs natural language supervision to learn better representations of binary code (i.e., assembly code) and get better transferability. At the core, our approach boosts superior transfer learning capabilities by effectively aligning binary code with their semantics explanations (in natural language), resulting a model able to generate better embeddings for binary code. To enable this alignment training, we then propose an efficient dataset engine that could automatically generate a large and diverse dataset comprising of binary code and corresponding natural language explanations. We have generated 195 million pairs of binary code and explanations and trained a prototype of CLAP. The evaluations of CLAP across various downstream tasks in binary analysis all demonstrate exceptional performance. Notably, without any task-specific training, CLAP is often competitive with a fully supervised baseline, showing excellent transferability. We release our pre-trained model and code at https://github.com/Hustcw/CLAP.

==> legancy.tex <==
\section{Methodology}
\label{sec:method}
%-------------------------------------------------------------------------------
Figure~\elsa{figure} illustrates the primary workflow presented in this paper, providing an overview of the key processes involved.

We performed numerous compilations using the Ubuntu source, resulting in assembly codes generated with various optimizations and compilers, while preserving the corresponding source codes. We acquired source code-level interpretations from GPT-3.5 as our bootstrap using appropriate prompts. We then fine-tuned LLaMA locally with the obtained data to align its output format with our needs and conducted local inference, yielding additional diversified code interpretations. Due to significant differences between the models and the use of distinct training data and alignment methods, text data enhancement was achieved. \wh{to be polished}

After attaining text descriptions corresponding to assembly code, we first pre-trained a jump-aware transformer on an extensive assembly code dataset to develop a well-expressive encoder model. Subsequently, using a contrastive learning approach featuring numerous negative samples, we aligned the assembly code encoder with a text encoder pre-trained on over 1 billion text pairs. By optimizing InfoNCE loss, we increased mutual information between positive and negative samples of assembly code and descriptions, ultimately matching the assembly code and text description and aligning their embeddings.

\subsection{Data Engine}

% 在这一个章节中，我们将介绍具体如何得到我们的用于进行预训练的数据，包括汇编代码、对应的源代码和源代码的LLM的解释。

In this section, we will discuss the process of obtaining pre-training data, which encompasses assembly code, corresponding source code, and the interpretation of the source code from LLM.

\subsubsection{Binary Generation}
\label{subsubsec:binary-generation}

% 我们借助于软件包管理器来实现大规模自动化的编译与源代码获取，我们使用Ubuntu的包管理器来完成这件事。

We utilize package managers to achieve large-scale automated compilation and source code acquisition, specifically using Ubuntu's package manager for this purpose. Ubuntu is one of the most popular distributions, containing over 30,000 packages, each with a compilation script that transforms the source code into the final product. This makes it suitable for generating a diverse set of binary executable files along with their corresponding source codes. 
% 在对Ubuntu包管理器的源代码进行编译的时候，我们替换了系统的编译器为我们的编译器forwarder，替换编译选项的部分为我们的所需要的，同时对涉及到的源代码文件进行记录，比如替换编译选项中的优化选项或者在即使是包管理器的工具调用了GCC时，仍然使用Clang来进行编译，以比设置CFLAGS和CC等环境变量更加高效与严格的方式来得到不同的优化等级和编译器。通过这种方式，我们得到了在汇编级别的增强。
% By replacing the system compiler with various compilers and optimization options within the Ubuntu source, we can attain assembly-level enhancements.

When compiling the source code for Ubuntu's package manager, we replaced the default system compiler with our custom compiler forwarder and adjusted the compilation options to meet our requirements such as altering optimization options within the compilation settings or employing \texttt{Clang} for compilation, even if the package manager's tool invoked \texttt{GCC}. This method proved to be more efficient and rigorous than merely configuring environment variables, such as \texttt{CFLAGS} and \texttt{CC}, to achieve diverse optimization levels and compilers.

% 为了能够得到相比起直接从原文件中得到更加精确的源代码对应关系，同时保留更多的变量名与宏定义名字中的语义信息，使得帮助LLM的源代码理解与解释。我们让编译器在编译的时候，让他omits directives like \texttt{ifdef} and \texttt{elseif}, maintains comments, and avoids macro expansion. Moreover, 在从最终得到的binary中的汇编代码得到对应的源代码是，it employs debug information to identify the actual source code addresses for each function in the binary, reducing problems caused by identically named functions within the same project. 
% 为了实现上面的目的，We use the \texttt{-E} option during compilation to obtain preprocessed source code, eliminating interference from \texttt{ifdef} and \texttt{elseif}.
% This method is more accurate and retains greater semantic information for the LLM as compared to decompiling from the binary. It prevents the expansion of semantic macro names, further assisting the LLM in understanding the source code.

In order to obtain more accurate source code correspondence compared to directly obtaining it from the original file, and to retain more semantic information in variable names and macro definition names compared to decompiling the assembly code to aid source code understanding and interpretation for LLM, we modify the compiler's behavior during compilation. Specifically, we instruct the compiler to omit directives like \texttt{ifdef} and \texttt{elseif}, maintain comments, and avoid macro expansion by adding \texttt{-E} option during compilation. Furthermore, when obtaining corresponding source code from the final binary's assembly code, it employs debug information to identify the actual source code addresses for each function in the binary, reducing problems caused by identically named functions within the same project.


\subsubsection{Source Code Description}

% To employ the GPT-3.5 model to interpret source code, we design the prompt with inspiration from CLIP's alignment capabilities. 我们将在subsection中提取的到的源代码，让GPT-3.5模型进行解释。在设计prompt过程中，我们让模型focuses on capturing an overview of the code's execution并且避免detailed step-by-step explanations.因为在测试过程中，我们观察到模型往往会主动地进行CoT，而在汇编层面往往比较难以获得这样子的信息。Additionally, we prevent output that includes variable names or other information这些不包含在stripped的binary中的信息. In our experiment, the model generated multiple tags to categorize the code segment.

To interpret source code using the GPT-3.5 model, we draw inspiration from CLIP's alignment capabilities when designing the prompt. We have the model analyze the extracted source code from the subsection. During the design process of the prompt for LLM, we ensure the model focuses on capturing an overview of the code's execution while avoiding detailed step-by-step explanations, which are often difficult to obtain at the assembly level. This is because, during testing, we observed that the model tended to naturally perform CoT\cite{weiChainThoughtPrompting2022} and yield verbose description. Additionally, we prevent output that includes variable names or other information not present in the stripped binary. At the last, we let the model generate multiple tags to categorize the code segment.

\subsubsection{Shadow Model}

We conduct supervised finetuning (SFT) on the LLaMA model using half of the 2.6 million function explanations from GPT-3.5, initializing it with the aligned Vicuña 13B model~\wh{cite vicuna and LLaMa} and performing complete finetuning to create a shadow model. For comparison, we train two additional models, one aligning LLaMA 13B and another aligning LLaMA 30B, both using 50,000 function explanations. We will evaluate and compare their performances in the following section.

Upon inspection, we discover that the Shadow Model, lacking a more in-depth RLHF, tends to output nonsensical results when faced with difficult source code. We notice that the corresponding perplexity is significantly larger compared to other, more typical models. Consequently, we eliminate the top 5\% of outputs with the highest perplexity across all models, determining that a perplexity of about 1.5 is a suitable threshold. \wh{we can enlarge this paragraph}

\subsubsection{Augmentation}

At the assembly level, we employ a variety of compilers and optimization levels to improve assembly code, which contains 6 different compilers (e.g \texttt{GCC-7}, \texttt{GCC-9}, \texttt{GCC-11}, \texttt{Clang-9}, \texttt{Clang-11} and \texttt{Clang-12}) and 5 optimization levels (e.g \texttt{O0}, \texttt{O1}, \texttt{O2}, \texttt{O3}, \texttt{Os}). Additionally, we maintain both stripped and non-stripped functions to facilitate assembly pre-training and contrastive pre-training in later stages. In terms of text interpretation, we harness the capabilities of both GPT-3.5 and our shadow model to generate distinct interpretations of each function, thereby enriching our analysis.

\subsection{Assembly Representation Model}
\subsubsection{Model Architecture}
\subsubsection{Pre-training}
\subsubsection{Contrastive Training}

